Detecting Emergent Intersectional Biases: Contextualized Word Embeddings Contain a Distribution of Human-like Biases

With the starting point that implicit human biases are reflected in the statistical regularities of language, it is possible to measure biases in English static word embeddings. State-of-the-art neural language models generate dynamic word embeddings dependent on the context in which the word appears. Current methods measure pre-defined social and intersectional biases that appear in particular contexts defined by sentence templates. Dispensing with templates, we introduce the Contextualized Embedding Association Test (CEAT), that can summarize the magnitude of overall bias in neural language models by incorporating a random-effects model. Experiments on social and intersectional biases show that CEAT finds evidence of all tested biases and provides comprehensive information on the variance of effect magnitudes of the same bias in different contexts. All the models trained on English corpora that we study contain biased representations. Furthermore, we develop two methods, Intersectional Bias Detection (IBD) and Emergent Intersectional Bias Detection (EIBD), to automatically identify the intersectional biases and emergent intersectional biases from static word embeddings in addition to measuring them in contextualized word embeddings. We present the first algorithmic bias detection findings on how intersectional group members are strongly associated with unique emergent biases that do not overlap with the biases of their constituent minority identities. IBD and EIBD achieve high accuracy when detecting the intersectional and emergent biases of African American females and Mexican American females. Our results indicate that biases at the intersection of race and gender associated with members of multiple minority groups, such as African American females and Mexican American females, have the highest magnitude across all neural language models.

==> 10_impact.tex <==
\iffalse
\section*{Broader Impact}
Outputs of neural language models trained on natural language expose their users to stereotypes and biases learned by such models. CEAT is a tool for analysts and researchers to measure social  biases in these models, which may help develop bias mitigation methods for neural language models. On the other hand, some users might utilize CEAT to detect certain biases or harmful stereotypes and accordingly target social groups by automatically generating large-scale biased text. Some users might generate and share biased content to shift public opinion as part of information influence operations. By focusing on the attitude bias measured by valence, a malicious actor might figure out ways to automatically generate hate speech while targeting certain social groups. 

In addition to the improper use of CEAT, another ethical concern is about IBD and UIBD: 
IBD and UIBD can detect  stereotypical associations for an intersectional group, but the detected words may be used in the generation of offensive content that perpetuates or amplifies existing biases.
Using the biased outputs of these neural language models leads to a feedback cycle when machine generated biased text ends up in training data contributing to perpetuating or amplifying bias.

\fi

==> old_main.tex <==


% \documentclass{article}

% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2020

% ready for submission
% \usepackage{neurips_2020}

% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
    % \usepackage[preprint]{neurips_2020}

% to compile a camera-ready version, add the [final] option, e.g.:
    % \usepackage[final]{neurips_2020}

% to avoid loading the natbib package, add option nonatbib:
    %  \usepackage[nonatbib]{neurips_2020}

% \usepackage[numbers]{natbib}
% \usepackage{neurips_2020}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{float}
\usepackage{booktabs} 
\usepackage{xcolor} 
\usepackage{graphicx}

\usepackage{multirow}
\usepackage{ragged2e}
\usepackage{amsmath}
% \usepackage[nodisplayskipstretch]{setspace}
% \setstretch{1.5}
% \usepackage[compact]{titlesec}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
% professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{enumitem}
\usepackage{xcolor,colortbl}

\clubpenalty = 10000
\widowpenalty = 10000
\displaywidowpenalty = 10000


\newcommand{\aylin}{{\textcolor{red}{Aylin: }} \textcolor{red} }
\newcommand{\wei}{{\textcolor{blue}{Wei: }} \textcolor{blue} }
\definecolor{lightgray}{rgb}{0.83, 0.83, 0.83}
\definecolor{darkgray}{rgb}{0.5, 0.5, 0.5}
\definecolor{mediumgray}{rgb}{0.66, 0.66, 0.66}


\title{Detecting Emergent Intersectional Biases: Contextualized Word Embeddings Contain a Distribution of Human-like Biases}
%\title{Quantifying Social Biases in Contextual Word Embeddings and Detecting Intersectional Biases in Static Word Embeddings \textcolor{red}{the title should be the summary of the research findings, contribution}}
\author{%
  % examples of more authors
%   \And
  Wei Guo \\
%   Department of Computer Science\\
  George Washington University\\
%   Washington, DC 20052 \\
  \texttt{weiguo@gwu.edu} \\
    Aylin Caliskan\\
  George Washington University\\
  \texttt{aylin@gwu.edu} \\
}


\begin{document}
\setlength{\textfloatsep}{\baselineskip }
\maketitle

\begin{abstract}
     \input{0_abstract}
\end{abstract}
%  \input{00_schedule}
 \input{1_intro}
 \input{2_problem}
 \input{3_related}
  \input{4_data}
 \input{5_approach}
 \input{6_experiments}
%  \input{7_results}
 \input{8_discussion}
 \input{9_conclusion}
 \input{10_impact}
%  \input{supp}
 
\bibliography{emnlp-ijcnlp-2019}
% \bibliographystyle{acl_natbib}
% \bibliographystyle{apa}
\bibliographystyle{unsrt}

% \input{supp/supp_1.tex}

\end{document}


==> t.tex <==
\begin{table*}[t]
\centering
\caption{
\textbf{CEAT for social and intersectional biases.} We report the overall magnitude of bias in a neural language model with CES$^{\ast}$ ($d$, rounded down) and its statistical significance with combined $p$-values ($p$, rounded up). CES pools $N = 10,000$ samples from a random-effects model.
    $Ci$ stands for the $i^{th}$ WEAT test in Table 1 from \cite{caliskan2017semantics}. $Ii$ stands for the tests constructed for intersectional biases. $A\_$ stands for African Americans. $E\_$ stands for European Americans. $M\_$ stands for Mexican Americans. $\_F$ stands for females. $\_M$ stands for males. Light, medium, and dark gray shading of combined $d$ values (CES) indicates small, medium, and large effect size respectively.  \textcolor{red}{I am not sure where these paranthesis are}
}
\label{table:socialbias-measure}
  {%
\begin{tabular}{|p{7mm} l |  r | cc | cc | cc |cc |}
\hline
\multicolumn{3}{| c |}{ \multirow{2}{*}{\textbf{Test}}} &
  \multicolumn{2}{c|}{\textbf{ELMo}} &
  \multicolumn{2}{c|}{\textbf{BERT}} &
  \multicolumn{2}{c|}{\textbf{GPT}} &
  \multicolumn{2}{c |}{\textbf{GPT-2}} \\ \cline{4-11} 
                          \multicolumn{3}{|c|}{}  & \textbf{$d$} & \textbf{$p$}  & \textbf{$d$} & \textbf{$p$}  & \textbf{$d$} & \textbf{$p$} & \textbf{$d$} & \textbf{$p$} \\ \hline
                                    
                                    
\multirow{2}{}{\shortstack{C1:}} &  Flowers/Insects  &     random       &  \cellcolor{darkgray}1.40       & $<10^{-30}$           & \cellcolor{darkgray}0.97       &  $<10^{-30}$            & \cellcolor{darkgray}1.04       & $<10^{-30}$          & 0.14       & $<10^{-30}$  \\

  &  Pleasant/Unpleasant$^{\ast}$    &        fixed            & \cellcolor{darkgray}{1.35}                     & $<10^{-30}$                     & \cellcolor{mediumgray}{0.64   }                  & $<10^{-30}$                     & \cellcolor{darkgray}{1.01       }               & $<10^{-30}$                     & \cellcolor{lightgray}{0.21     }                 & $<10^{-30}$                     \\ \hline



\multirow{2}{}{{\shortstack{C2:}}} & Instruments/Weapons &     random     & \cellcolor{darkgray}1.56       & $<10^{-30}$           & \cellcolor{darkgray}0.94       & $<10^{-30}$  & \cellcolor{darkgray}1.12       & $<10^{-30}$          & \cellcolor{lightgray}-0.27      & $<10^{-30}$      \\
 &  Pleasant/Unpleasant$^{\ast}$    &        same           & \cellcolor{darkgray}{1.59}                     & $<10^{-30}$                     & \cellcolor{mediumgray}{0.54}                     & $<10^{-30}$                     & \cellcolor{darkgray}{1.09}                     & $<10^{-30}$                     & \cellcolor{lightgray}{-0.21 }                    & $<10^{-30}$  \\ \hline
 
 \multirow{2}{}{{\shortstack{C3:}}} & EA/AA names &     random     & \cellcolor{lightgray}0.49       & $<10^{-30}$  & \cellcolor{lightgray}0.44       & $<10^{-30}$   & -0.11      & $<10^{-30}$       & -0.19      & $<10^{-30}$      \\
 &  Pleasant/Unpleasant$^{\ast}$    &        same           & \cellcolor{lightgray}{0.47  }                   & $<10^{-30}$                     & \cellcolor{lightgray}{0.31}                     & $<10^{-30}$                     & -0.10                    & $<10^{-30}$                     & 0.09                      & $<10^{-30}$     \\ \hline
 
  \multirow{2}{}{{\shortstack{C4:}}} & EA/AA names &     random     & 0.15       & $<10^{-30}$  & \cellcolor{lightgray}0.47       & $<10^{-30}$  & 0.01       & $<10^{-2}$       & \cellcolor{lightgray}-0.23      & $<10^{-30}$      \\
 &  Pleasant/Unpleasant$^{\ast}$    &        same           & \cellcolor{lightgray}{0.23 }                    & $<10^{-30}$                     & \cellcolor{lightgray}{0.49 }                    & $<10^{-30}$                     & 0.00                     & $0.20$                          & -0.13                     & $<10^{-30}$     \\ \hline
 
  \multirow{2}{}{{\shortstack{C5:}}} & EA/AA names &     random     & 0.11       & $<10^{-30}$   & 0.02       & $<10^{-7}$        & 0.07       & $<10^{-30}$  & \cellcolor{lightgray}-0.21      & $<10^{-30}$      \\
 &  Pleasant/Unpleasant$^{\ast}$    &        same           & 0.17                     & $<10^{-30}$                     & 0.07                     & $<10^{-30}$                     & 0.04                     & $<10^{-27}$                     & -0.01                     & 0.11        \\ \hline 
 
   \multirow{2}{}{{\shortstack{C6:}}} & Males/Female names &     random     & \cellcolor{darkgray}1.27       & $<10^{-30}$            & \cellcolor{darkgray}0.92       & $<10^{-30}$  & 0.19       & $<10^{-30}$  & \cellcolor{lightgray}0.36       & $<10^{-30}$     \\
 &  Career/Family    &        same           & \cellcolor{darkgray}{1.31  }                   & $<10^{-30}$                     & \cellcolor{lightgray}{0.41}                     & $<10^{-30}$                     & 0.11                     & $<10^{-30}$                     & \cellcolor{lightgray}{0.34}                      & $<10^{-30}$        \\ \hline 
 
    \multirow{2}{}{{\shortstack{C7:}}} & Math/Arts &     random     & \cellcolor{mediumgray}0.64       & $<10^{-30}$   & \cellcolor{lightgray}0.41       & $<10^{-30}$  & \cellcolor{lightgray}0.24       & $<10^{-30}$  & -0.01      & $<10^{-2}$      \\
 &  Male/Female terms    &        same           & \cellcolor{darkgray}{0.71 }        &                 $<10^{-30}$              & \cellcolor{lightgray}{0.20  }                   & $<10^{-30}$                     & \cellcolor{lightgray}{0.23}                     & $<10^{-30}$                     & -0.14                     & $<10^{-30}$          \\ \hline 
 
 \multirow{2}{}{{\shortstack{C8:}}} & Science/Arts &     random     & \cellcolor{lightgray}0.33       & $<10^{-30}$   & -0.07      & $<10^{-30}$        & \cellcolor{lightgray}0.26       & $<10^{-30}$  & -0.16      & $<10^{-30}$     \\
 &  Male/Female terms    &        same           & \cellcolor{mediumgray}{0.51     }                & $<10^{-30}$                     & 0.17                     & $<10^{-30}$                     & \cellcolor{lightgray}{0.35}                     & $<10^{-30}$                     & -0.05                     & $<10^{-30}$              \\ \hline 
 
  \multirow{2}{}{{\shortstack{C9:}}} & Mental/Physical disease &     random     & \cellcolor{darkgray}1.00       & $<10^{-30}$   & \cellcolor{mediumgray}0.53       & $<10^{-30}$  & 0.08      & $<10^{-29}$       & 0.10       & $<10^{-30}$     \\
 &  T/P    &        same           & \cellcolor{darkgray}{1.01}                     & $<10^{-30}$                     & \cellcolor{lightgray}{0.40}                     & $<10^{-30}$                     & \cellcolor{lightgray}{-0.23 }                   & $<10^{-30}$                     & \cellcolor{lightgray}{-0.21 }                    & $<10^{-30}$               \\ \hline 
 
   \multirow{2}{}{{\shortstack{C10:}}} & Young/Old people's names &     random           & 0.11       & $<10^{-30}$  & -0.01       & 0.016        & 0.07       & $<10^{-30}$       & -0.16      & $<10^{-30}$     \\
 &  P/U    &        same           & \cellcolor{lightgray}{0.24}                     & $<10^{-30}$                     & 0.07                     & $<10^{-30}$                     & 0.04                     & $<10^{-17}$                     & -0.14                     & $<10^{-30}$          \\ \hline 
 
    \multirow{2}{}{{\shortstack{I1:}}} & AF/EM names &     random           & \cellcolor{darkgray}1.24       & $<10^{-30}$            & \cellcolor{mediumgray}0.77       & $<10^{-30}$   & 0.07       & $<10^{-30}$  & 0.02       & $<10^{-2}$     \\
 &  AF/EM intersectional    &        same           & \cellcolor{darkgray}{1.25}                    & $<10^{-30}$                    & \cellcolor{darkgray}{0.98  }                  & $<10^{-30}$                      & \cellcolor{lightgray}{0.23  }                   & $<10^{-30}$                     & -0.19                     & $<10^{-30}$         \\ \hline 
 
     \multirow{2}{}{{\shortstack{I2:}}} & AF/EM names &     random           & \cellcolor{darkgray}1.25      & $<10^{-30}$            & \cellcolor{mediumgray}0.67      & $<10^{-30}$   & -0.09      & $<10^{-30}$      & 0.02       & $<10^{-2}$    \\
 &  AF emergent/EM intersectional    &        same           & \cellcolor{darkgray}{1.27} & $<10^{-30}$ & \cellcolor{darkgray}{1.00} & $<10^{-30}$                     & \cellcolor{lightgray}{0.23   }                  & $<10^{-30}$                     & -0.14                     & $<10^{-30}$         \\ \hline 
 
      \multirow{2}{}{{\shortstack{I3:}}} & MF/EM names &     random           & \cellcolor{darkgray}1.31       & $<10^{-30}$            & \cellcolor{mediumgray}0.68       & $<10^{-30}$   & -0.06       & $<10^{-30}$      & \cellcolor{lightgray}0.38       & $<10^{-30}$    \\
 &  MF/EM intersectional    &        same           & \cellcolor{darkgray}{1.29}& $<10^{-30}$ & \cellcolor{mediumgray}{0.51} & $<10^{-30}$                     & 0.00                     & 0.81                            & \cellcolor{lightgray}{0.32  }                    & $<10^{-30}$          \\ \hline 
 
       \multirow{2}{}{{\shortstack{I4:}}} & MF/EM names &     random           & \cellcolor{darkgray} 1.51       & $<10^{-30}$           &\cellcolor{darkgray} 0.86      & $<10^{-30}$  & 0.16       & $<10^{-30}$  & \cellcolor{lightgray}-0.32      & $<10^{-30}$    \\
 &  MF emergent/EM intersectional  &         same           & \cellcolor{darkgray}{1.43} & 
 $<10^{-30}$ & \cellcolor{mediumgray}{0.58} & $<10^{-30}$ & \cellcolor{lightgray}{0.20} & $<10^{-30}$ & \cellcolor{lightgray}{-0.25} & $<10^{-30}$        \\ \hline 

\end{tabular}
}
\end{table*}
